Maximum A Posteriori Ly-alpha Estimator (MAPLE): Band-power and covariance estimation of the 3D Ly-alpha forest power spectrum

We present a novel maximum a posteriori estimator to jointly estimate band-powers and the covariance of the three-dimensional power spectrum (P3D) of Lyman-alpha forest flux fluctuations, called MAPLE. Our Wiener-filter based algorithm reconstructs a window-deconvolved P3D in the presence of complex survey geometries typical for Lyman-alpha surveys that are sparsely sampled transverse to and densely sampled along the line-of-sight. We demonstrate our method on idealized Gaussian random fields with two selection functions: (i) a sparse sampling of 30 background sources per square degree designed to emulate the currently observing the Dark Energy Spectroscopic Instrument (DESI); (ii) a dense sampling of 900 background sources per square degree emulating the upcoming Prime Focus Spectrograph Galaxy Evolution Survey. Our proof-of-principle shows promise, especially since the algorithm can be extended to marginalize jointly over nuisance parameters and contaminants, i.e.offsets introduced by continuum fitting. Our code is implemented in JAX and is publicly available on GitHub.

==> cut_section.tex <==

\subsection{Constraining power vs. P1D}

To demonstrate the relative cosmological constraining power of the three dimensional Lyman Alpha forest to the standard 1D analysis we perform a Markov Chain Monte Carlo cosmological analysis with both methods using the same data. We will focus our analysis on the standard cosmological parameters $A_s$, $n_s$, and $Omega_m$, as well as the hydrodynamically motivated parameters from Equation \ref{eq:eq:dkmu}, $k_p$ and $\alpha_p$.


We note that this method is a somewhat circuitous as, given a differentiable model for the three dimensional flux (i.e. a differentiable version of Eq. \ref{eq:p3d}) we can perform the MUSE analysis in terms of the underlying cosmological parameters rather than the band-powers. This would greatly simplify the overall numerical analysis, but construct a model dependant result. For this particular model it isn't currently computationally feasible to perform direct parameter inference due to difficulty in creating a differentiable Boltzmann code to compute derivatives of $P_L(k)$. 

For our likelihood model, we use the estimated covariance found via Equation \ref{eq:H} and \ref{eq:J}. We set up a mean squared log-likelihood model for the set of model parameters $\Theta = \{A_s/A_{fid},n_s, \Omega_m,k_p,\alpha_p\}$ as
\begin{equation}
    \mathcal{L}(\Theta|\theta) = (\theta_i - P_{L,F}(\Theta)_i) \Sigma_{ij}^{-1}(\theta_j - P_{L,F}(\Theta)_j) + \text{Prior}(\Theta),
\end{equation}
where for the prior term we choose a Gaussian centered on the model true value with standard deviation $\sigma_\Theta = \{0.02,0.1,0.1,0.2,0.6\}.$

Comparing to P1D
We can map our theoretical model to P3D via;

\begin{equation}
    P_{\textrm 1D}(k_\parallel) = \frac{1}{2\pi} \int_{k_\parallel}^\infty dk kP_{\textrm 3D}(k,k_\parallel)
\end{equation}
\label{subsec:analysis_DLA}



%$O_i$, drawn from $\mathcal{N}(0,\sigma^2_F)$, where $\sigma_F$ is the standard deviation of the mean flux over lines of sight in the survey. In general, this distribution could be calibrated from a simulation or inferred from the data itself, but for the purpose of this work we will assume a known $\sigma_F = 0.1$. 
%To our latent space vector containing the phase information we append additional values of the mean flux offest, $\{O_1, \cdots, O_i, \cdots, O_N\}$, for $N$ observed lines of sight. With this new latent space vector, we can perform the same analysis as described in Sec. \ref{subsec:muse}.


%%%%%%%%%%%%


\section*{Appendix: Joint marginalization over systematic}


The MUSE framework is flexible to additional systematics as their associated nuisance parameters as they can be treated as latent space parameters (like the phases) for marginalization. A common systematic/uncertainty in \lya\ studies is the mean flux in the \lya\ forest region. In most studies the overall fitted continuum is re-scaled such that the mean flux of the region is that from simulations and/or observations. However, this analysis disregards cosmological information found in the spatially varying nature of the underlying flux field. In the sections, we will add onto the analysis of Sec. \ref{subsec:hydro} the inclusion of this mean flux offset.

We choose a simple model, following work in \cite{2018Krolewski,2019TARDISI,2021TARDISII} for the unresolved mean flux where we apply a multiplicative offset to the observed flux
\begin{equation}
    F_\textrm{obs} = \frac{F_\textrm{sim}}{1+\delta_c},
\end{equation}
where $\delta_c$ is taken from an underlying normal distribution, $\mathcal{N}(0,\sigma^2_c(\rm{S/N}))$. The dependence of the variance from the signal to noise is due to the increased uncertainty in continuum fitting in the noisy regime. We can model the dependence on signal to noise as 
\begin{equation}
 \sigma_c = \frac{0.205}{\rm{S/N}} + 0.015,
\end{equation}
where the constants come from the CLAMATO survey \citep{2018CLAMATO1}, which include both QSOs and LBGs. To our latent space vector we append additional values of the mean flux factor, $\{O_1, \cdots, O_i, \cdots, O_N\}$, for $N$ observed lines of sight. With this new latent space vector, we can perform the same analysis as described in Sec. \ref{subsec:muse}. For simplicity, we simplify our fiducial power spectrum from Eq. \ref{eq:p3d} by setting $D(k,\mu)=1$ (i.e. only including the Kaiser term). This allows us to just fit $P_L(k)$ as opposed to a full two dimensional binned quantity, clarifying the exposition and computation for demonstration purposes.

We perform the fit both with and without including a continuum offset term and show the resulting power spectra and associated errors in Figure \ref{fig:offset_pk}. While including the continuum offset term, we find less constraining power at larger scales ($k < 0.02$) but near identical constraints at smaller scales ($k>0.05$). This can be understood as the presence of continuum offsets effecting the largest scale modes, which in turn effect adjacent modes due to the survey geometry. We can see this visually by the difference in estimated covariance matrices, shown in Figure \ref{fig:offset_covariance}.

\roger{we should discuss this section: Make it more explicit what implications this has - which can be quite interesting. Keeping large-scale modes in the continuum fit introduces quite a bit of noise given current continuum reconstruction techniques. Thus, having means to marginalize over uncertainties in our continuum fit is powerful...}

\begin{figure}
    \centering
    \includegraphics[scale=0.65]{offset_pk.pdf}
    \caption{Offset power spectra}
    \label{fig:offset_pk}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[scale=0.65]{covariance_offset.pdf}
    \caption{Difference in covariance matrix between including continuum offsets and without continuum offsets. As expected, the presence of continuum offsets effects the reconstruction of largest scale modes which then effect the reconstruction of smaller scales (due to the survey window function effects). \roger{Great - to what scales does the bin index translate? And the colorbar is unclear to me. Perhaps you can make it a correlation matrix or PTE or something slightly more intuitive.}}
    \label{fig:offset_covariance}
\end{figure}


%%%%%%%%


\begin{figure}
    \centering
    \includegraphics[scale=0.65]{p1d.pdf}
    \caption{Projection of the reconstructed band powers to the standard one dimension. For estimated errors, we take the linear combination of the associated band-powers. Note this may underestimate errors in the presence of strong off-diagonal elements and shouldn't be used instead of the original 2d estimated quantity for likelihood analysis.}
    \label{fig:p1d}
\end{figure}
